MAFALDA: A Benchmark and Comprehensive Study of Fallacy Detection and Classification

We introduce MAFALDA, a benchmark for fallacy classification that merges and unites previous fallacy datasets. It comes with a taxonomy that aligns, refines, and unifies existing classifications of fallacies. We further provide a manual annotation of a part of the dataset together with manual explanations for each annotation. We propose a new annotation scheme tailored for subjective NLP tasks, and a new evaluation method designed to handle subjectivity. We then evaluate several language models under a zero-shot learning setting and human performances on MAFALDA to assess their capability to detect and classify fallacies.

==> MAFALDA_arXiv_-_Copie/src/abstract.tex <==
We introduce MAFALDA, a benchmark for fallacy classification that merges and unites previous fallacy datasets. It comes with a taxonomy that aligns, refines, and unifies existing classifications of fallacies. We further provide a manual annotation of a part of the dataset together with manual explanations for each annotation. We propose a new annotation scheme tailored for subjective NLP tasks, and a new evaluation method designed to handle subjectivity.
We then evaluate several language models under a zero-shot learning setting and human performances on MAFALDA to assess their capability to detect and classify fallacies.


==> MAFALDA_arXiv_-_Copie/src/annotation.tex <==
\section{Tackling Subjectivity in Annotations}\label{sec:annot_dataset}




\subsection{Subjectivity in Fallacy Annotation}\label{sec:subjectivity}

Annotating fallacies is an inherently subjective endeavor. 
To see this, consider Example (c) in Figure~\ref{fig:main}.
The argument goes that the candidate has to win again because he won last time. This can be seen as a \emph{false causality} fallacy: a cause-effect relationship is incorrectly inferred between two events that have nothing to do with each other.
However, it can also be seen as a \emph{causal oversimplification} fallacy. This is because
we can contend that having won the last election gives the candidate an edge over other candidates in terms of visibility, and thus makes it more likely that he wins this year's election as well. The argument is thus fallacious mainly because it fails to acknowledge other factors that play a role in re-election.

This simple example already shows subjectivity in fallacy annotations, where several annotations can be defended. It would be counter-productive if the annotators converged on, say, \emph{causal oversimplification}, so that every approach of fallacy annotation is penalized for proposing an (equally plausible) \emph{false causality}. There are other cases of legitimately differing opinions: One annotator may see implicit assertions that another annotator does not see. In ``\textit{Are you for America? Vote for me!}'' one reader may see the implicit ``\textit{or you must be against America}'' (which makes this a \emph{false dilemma}), while another annotator may see no such implicature. Annotators may also have different thresholds for fear (\emph{appeal to fear}) or insults (\emph{ad hominem}). 
Finally, different annotators have different background knowledge: A sentence such as ``\textit{Use disinfectants or you will get Covid-19!}'' 
may be read as a plausible warning by one annotator but as an \emph{appeal to fear} fallacy by an annotator who knows that Covid-19 does not spread via contaminated surfaces. 
We will now present a disjunctive annotation scheme that accounts for this inherent subjectivity.


%




\input{src/evaluation_metric}








\section{MAFALDA Dataset}\label{sec:dataset}


\subsection{Source Datasets}\label{sec:dataset:sources}

We used four publicly available fallacy datasets to construct our benchmark:







We imported all 8,576 texts from \citet{sahaiBreakingInvisibleWall2021}. These are online discussions from Reddit, as in Example~(d) of Figure~\ref{fig:main}. %
We reconstructed the texts by concatenating the post of interest, the previous post (if available), and the title. The title was considered as a citation and was thus not annotated. This dataset contains sentences that were labeled as negative examples.

We imported all 336 texts from \citet{martinoFineGrainedAnalysisPropaganda2019}, which are from news outlets.
We imported all 583 texts from \citet{jinLogicalFallacyDetection2022}, which are either toy examples gathered from online quizzes (as in Example~(a)), or longer climate-related texts originating from news outlets.
Finally, we imported all 250 texts from \citet{goffredoFallaciousArgumentClassification2022}, which are American political debates (Example~(b)). 
We split these longer texts into shorter texts by concatenating the previous and following sentences of allegedly fallacious texts. 

\textbf{This gives us an English-language corpus of 9,745 texts, which is diverse in terms of linguistic terms and text length.} 
We removed URLs, emails, and phone numbers globally. 




\subsection{Annotation}\label{sec:annotation:annotation}

The existing annotation schemes on our corpus varied a lot among papers: 
 %
for example, only \citet{sahaiBreakingInvisibleWall2021} approached the annotation task as a binary classification, where annotators determine if a given text contains a specified type of fallacy.
The annotations process also varied greatly w.r.t. how consensus was obtained, as explained in Section~\ref{subsec:subjectivity}.

Therefore, we removed all annotations, and manually re-annotated, from scratch, 200 randomly selected texts from our merged corpus. Our sample mirrors the distribution of sources and the original labels in our corpus: it contains 124 texts from \citet{sahaiBreakingInvisibleWall2021}, 59 texts from \citet{jinLogicalFallacyDetection2022}, and 17 political debate texts from \cite{goffredoFallaciousArgumentClassification2022}.
We did not use the texts from \citet{martinoFineGrainedAnalysisPropaganda2019} we initially planned to use because they were more than 5,000 characters long.
Thus, annotating a single text would considerably bias the work towards Martino’s. However, the texts are part of our cleaned and homogenized dataset, and our goal is to include the annotations of these texts as we enlarge our manual annotation.


\textbf{LLMs were not involved} in the annotation process. We did \textbf{not involve crowd workers} either, because  
~33\%-46\% of Mturk workers are estimated to use ChatGPT~\cite{veselovsky2023artificial}. %
Hence, we annotated the texts ourselves.
Our task was (\textit{i}) identifying each argument in a text, (\textit{ii}) determining whether it is fallacious, (\textit{iii}) determining the span of the fallacy (as defined in Definition~\ref{def:span}), and (\textit{iv}) choosing the fallacy type(s).
We discussed each fallacious span together, and either converged on one annotation or permitted several alternative annotations for the same span. 
\textbf{We provide an explanation for each annotation}, and \textbf{we provide a completed template for each annotation}, as defined in Section~\ref{sec:tax}. 
For instance, 
Example (d) from Figure~\ref{fig:main}, which shows an \emph{appeal to ridicule}: the post argues against the possibility of working in finance with a law degree by exaggerating the position and thus portraying it as ridicule. Breaking down the example with the formal definition yields:
\begin{itemize}[noitemsep,nolistsep,leftmargin=4mm]
    \item $E_1$= The original poster
    \item $P$= It might be possible to work in finance with a law degree
    \item $E_2$= The author of the post.
    \item $P'$= Law school students are so intelligent that they can do any job, even surgeons.
\end{itemize}
Here, $E_i$ are entities (persons, organizations) or groups of entities, $P$ and $P'$ are premises, properties, or possibilities. %


The process took around 40 hours.
This corresponds to an average of 12 minutes per example, ranging from less than a minute for toy examples to half an hour when disagreement raised a debate. The total number of person-hours was 130.
Details about the annotators can be found in Appendix~\ref{app:annotators}.



\subsection{Statistics}

Our dataset comprises 9,745 texts, of which 200 texts have been annotated manually, with a total of 268 spans. 
Among these, 137 texts contained at least one span identified as fallacious,
while the remaining texts did not contain any fallacious spans.
The mean number of spans per text is 1.34. 

Among the 200 texts, 71 were initially labeled as non-fallacious.
However, our annotation found fallacies in some of these texts. This can be explained by the methodology from \citet{sahaiBreakingInvisibleWall2021}, where crowd workers check only one specific type of fallacy. If that fallacy is not present, the text is annotated as non-fallacious. Our annotation, however, spotted other fallacies in the text, and labeled them. 
In the end, we have 63 non-fallacious texts. 





The dataset contains all the fallacies presented in Section~\ref{sec:tax}.
The three most frequent fallacies represent 1/4 of the dataset, while the least frequent fallacies appear less than three times. \textbf{71.5\% of the texts were annotated with a similar fallacy as the original one} (at least one fallacy of the source annotation was in the new annotation, or we agreed on a non-fallacious text). The difference is mainly because our taxonomy introduced new fallacies, such as \emph{appeal to ridicule}, and removed fallacies that we considered too vague or broad, such as \emph{intentional fallacy}. 
In some cases, we used a different granularity than in the source: while the source might say \emph{appeal to emotion}, we annotated, e.g., with \emph{appeal to fear}. We also permit several alternative annotations per span, which entails that the new annotations have, on average, more annotations per text than the source annotations (Original: 0.665, Ours: 1.34). 






The dataset contains 203 spans, of which 65 
(i.e.,~28\%) contain at least two different (alternative) labels (see Example~\ref{ex:main}).
We computed the co-occurrence matrix of the fallacies.
Most fallacies do not co-occur too frequently (less than 30\% of the time) with another particular fallacy, which indicates that \textbf{our definitions of fallacies are broadly orthogonal}. 
However, there are two fallacies with high co-occurrence frequency: \appealtopity~ has a 100\% co-occurrence with \strawman~ and \appealtoworseproblem. However, this is because there is only one occurrence of \appealtopity~ in our dataset. The second one is \guiltbyassociation, which is 38\% of the time associated with \adhominem. This is explained by the fact that \guiltbyassociation~ and \adhominem{} are two types of the \emph{ad hominem} fallacy.
Complete statistics about our dataset are provided in Appendix~\ref{app:dataset}.




==> MAFALDA_arXiv_-_Copie/src/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
We have presented MAFALDA, a unified dataset designed for fallacy detection and classification. This dataset integrates four pre-existing datasets into a cohesive whole, achieved through developing a new, comprehensive taxonomy. This taxonomy aligns %
publicly available taxonomies dedicated to fallacy detection. 
We manually annotated 200 texts from our dataset and provided an explanation in the form of a completed template for each of them. 
The disjunctive annotation scheme we proposed embraces the subjectivity of the task and allows for several alternative annotations for the same span. 
We have further demonstrated the capabilities of various large language models in zero-shot fallacy detection and classification at the span level.
While Level 0 classification shows good results, Levels 1 and 2 are largely out of reach of LLMs in zero-shot settings.
We hope that our benchmark will enable researchers to improve the results of this challenging task.

Future work includes expanding into few-shot settings and exploring advanced prompting techniques, such as chain-of-thought, using the template-based definitions of fallacy and the taxonomy we provided. Furthermore, we believe that using a top-down approach, i.e.,~from Level 0 to Level 2 of our taxonomy, may provide better results than the bottom-up approach we used in our experiments. 
Regarding our disjunctive annotation scheme, we are interested in exploring its use in other NLP domains.
Lastly, we plan to enrich the dataset with more annotated examples for model fine-tuning.\\

\textbf{Acknowledgement.} This work was partially funded by the NoRDF project (ANR-20-CHIA-0012-01), the SINNet project (ANR-23-CE23-0033-01) and Amundi Technology.






==> MAFALDA_arXiv_-_Copie/src/definitions.tex <==
\section{A Unified Taxonomy of Fallacies}\label{sec:def}



\subsection{Definitions}


We start with the definition of an argument, following \citet{copi2018introduction,britannica}:







\begin{mydef}[label={def:arg}]{Argument}
An argument consists of an assertion called the \emph{conclusion} and one or more assertions called \emph{premises}, where the premises are intended to establish the truth of the conclusion.
Premises or conclusions can be implicit in an argument.
\end{mydef}

\noindent Thus, an argument is typically of the form ``\textit{\textbf{Premise$_1$:} All humans are mortal. \textbf{Premise$_2$:} Socrates is human. \textbf{Conclusion:} Therefore, Socrates is mortal.}''. 
However, premises and conclusion can also appear in the opposite order and/or in the same sentence, as in ``\textit{Socrates is mortal because he is a human and all humans are mortal}''. 
In many real-world arguments, the premise and the conclusion are spread apart (as in ``\textit{Of course, Socrates is mortal! How can you doubt this? After all, he's human, and all humans are mortal!}''). Sometimes, premises are left implicit (as in ``\textit{Socrates is mortal because he is human}''). Even the conclusion can be implicit (as in ``\textit{Socrates is human and all humans are mortal}''). 
In the context of a discussion, an argument can attack another argument~\cite{dungAcceptabilityArgumentsIts1995}, in which case the conclusion is implicitly negated (``\textit{Socrates is immortal! -- But he is human!}''). 


A valid argument is one where the truth of the premises guarantees the truth of the conclusion; otherwise, following \citet{copi2018introduction, britannica}, the argument is a fallacy:
\begin{mydef}[label={def:fallacy}]{Fallacy}
A fallacy is an argument where the premises do not entail the conclusion. %
\end{mydef}
\noindent We refer the reader to \citet{tina} for a discussion of a formal definition of textual entailment. Appendix~\ref{sec:edge} further distinguishes fallacies from other types of erroneous statements. %







==> MAFALDA_arXiv_-_Copie/src/error_analysis.tex <==
\section{Error Analysis} \label{app:error_analysis}
We conduct an error analysis on two models, GPT-3.5 and Falcon, which exhibit the best and worst performance on Level 2. Our analysis also includes the annotations of the users study. \textbf{Our first goal in this analysis is to compare whether the best model has better controlled behavior than the worst model when generating outputs}. The Falcon model identifies 625 fallacious spans, with an average of 4.8 fallacies per span, while the GPT-3.5 model detects only 199 fallacious spans, with an average of 1.07 fallacies per span. However, we have 203 fallacious spans in the gold standard. 
The distribution of fallacies for the fallacious span at Level~2 for each model is presented in Table~\ref{tab:distribution_fallacies_level_2}. Based on our analysis, we have observed that the Falcon model tends to predict multiple fallacies that are irrelevant to a fallacious span.
In contrast, the GPT-3.5 model displays a more controlled behavior, which explains why Falcon has a low precision score. It is also worth noting that GPT-3.5 never predicted a span as \emph{tu quoque}.
We observe that both models produce nonsensical outputs, such as SQL code like ``\textit{select name color order from tag where the name},'' or incomplete classification of fallacies such as ``\textit{the sentence it's a mistake being considered as part of a fallacious argument.}''. Falcon has 115 spans labeled as unknown, while GPT-3.5 has only 5.  \textbf{Our second goal in this analysis is to analyze the exact matching performance of detecting fallacies and the type of fallacies that models and humans struggle with at Level~1}. Out of the 625 fallacious spans identified by Falcon, only 60 match the gold standard exactly, while out of 199 fallacious spans detected by GPT-3.5, only 55 match the gold standard exactly. Both models struggle mainly with fallacies categorized as fallacies of emotion, as shown in Figure~\ref{fig:correct_fallacy_models_level_1}.\\
For the annotators of the user study, we use a small sample of 20 examples with 24 spans. User 2 performs the best with 17 exactly matched spans, while User 4 performs worst with only 8 exactly matched spans. Based on the exact matched results, the analysis of Figure \ref{fig:correct_fallacy_users_level_1} reveals that all the annotators struggle mainly with the fallacies of 
 appeal to emotion. This difficulty can be partly attributed to these fallacies being less prevalent in our sample compared to the other types of fallacies. Interestingly, Users 1 and 3 correctly predict more fallacies of logic. Conversely, Users 2 and 4 correctly predict more fallacies of credibility than the others. It is worth noting that none of the users used all 23 fallacies of the taxonomy during the annotations, as shown in Table~\ref{tab:users_distribution_fallacies_level_2}.\\
In conclusion, models and humans tend to struggle more with fallacies of appeal to emotion, which could be expected since not every expression of emotion is necessarily a fallacy. The difficulty of the task lies in distinguishing valid arguments accompanied by emotions from fallacious arguments. 
This is supported by Figures~\ref{fig:correct_fallacy_models_level_1} and \ref{fig:correct_fallacy_users_level_1}. Despite the underrepresentation of the fallacies of the appeal to emotion in our user study sample, our findings indicate that humans often fail to exactly identify the specific fallacious spans classified under appeal to emotion fallacies. Moreover, even when humans correctly identify such fallacious spans, they are frequently misclassified. In contrast, models tend more to find these fallacious spans although they, too, frequently misclassify them. The only instances where the models can correctly predict the fallacious spans and their labels are when they involve an \emph{appeal to ridicule} or an \emph{appeal to a worse problem}. These cases can be observed in Figures~\ref{fig:correct_fallacy_models_level_2}.



\begin{table*}[ht]
\centering
\label{tab:fallacyComparison}
\begin{tabular}{@{}lccc@{}}
\toprule
Fallacy Type & Best Model & Worst Model & Gold Standard \\ \midrule
Appeal to Positive Emotion & 3 & 128 & 3 \\
Appeal to Anger & 6 & 119 & 6 \\
Appeal to Fear & 5 & 132 & 11 \\
Appeal to Pity & 1 & 198 & 1 \\
Appeal to Ridicule & 10 & 121 & 20 \\
Appeal to Worse Problems & 21 & 157 & 8 \\
Causal Oversimplification & 6 & 81 & 23 \\
Circular Reasoning & 8 & 132 & 11 \\
Equivocation & 1 & 106 & 7 \\
False Analogy & 6 & 127 & 12 \\
False Causality & 9 & 57 & 13 \\
False Dilemma & 6 & 169 & 18 \\
Hasty Generalization & 41 & 123 & 28 \\
Slippery Slope & 10 & 77 & 11 \\
Straw Man & 6 & 135 & 13 \\
Fallacy of Division & 2 & 102 & 2 \\
Ad Hominem & 32 & 135 & 16 \\
Ad Populum & 4 & 75 & 14 \\
Appeal to (False) Authority & 10 & 211 & 9 \\
Appeal to Nature & 7 & 143 & 11 \\
Appeal to Tradition & 4 & 156 & 6 \\
Guilt by Association & 4 & 91 & 8 \\
Tu Quoque & 0 & 111 & 3 \\
Unknown & 5 & 115 & - \\ \bottomrule
\end{tabular}
\caption{Fallacy distribution at Level 2 of the Gold standard, Best model and Worst model }
\label{tab:distribution_fallacies_level_2}
\end{table*}

\begin{table*}[ht]
\centering
\label{tab:fallacyComparison}
\begin{tabular}{@{}lccc@{}}
\toprule
Fallacy Type & Best Model & Worst Model & Gold Standard \\ \midrule
Emotion & 46 & 855 & 49 \\
Logic & 95 & 1109 & 138 \\
Credibility & 61 & 922 & 67 \\
Unknown & 5 & 115 & 0 \\ \bottomrule
\end{tabular}
\caption{Fallacy distribution at Level 1 of the Gold standard, Best model and Worst model }
\label{tab:distribution_fallacies_level_1}
\end{table*}



\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_best model_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{best model}}
        \label{fig:correct_fallacy_best_model_level_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_worst model_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{worst model}}
        \label{fig:correct_fallacy_worst_model_level_1}
    \end{subfigure}

    \caption{
    Accuracy of fallacy labeling for spans that \textbf{exactly match} the gold standard at Level 1 for the best and worst models. \emph{Exact Span} corresponds to the number of spans correctly identified by the model, \emph{Exact Span and Correct Label} corresponds to the number of correctly labeled spans out of the correctly identified spans.
    }
    \label{fig:correct_fallacy_models_level_1}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_best model_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{best model}}
        \label{fig:correct_fallacy_best_model_level_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_worst model_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{worst model}}
        \label{fig:correct_fallacy_worst_model_level_2}
    \end{subfigure}

    \caption{Accuracy of fallacy labeling for spans that \textbf{exactly match} the gold standard at Level 2 for the best and worst models. \emph{Exact Span} corresponds to the number of spans correctly identified by the model, \emph{Exact Span and Correct Label} corresponds to the number of correctly labeled spans out of the correctly identified spans.}
    \label{fig:correct_fallacy_models_level_2}
\end{figure*}

\begin{table*}[ht]
\centering

\begin{tabular}{@{}lccccc@{}}
\toprule
Fallacy Type & User 1 & User 2 & User 3 & User 4 & Sample Gold Standard \\ \midrule
Appeal to Positive Emotion & 2 & 0 & 0 & 2 & 0 \\
Appeal to Anger & 1 & 0 & 0 & 0 & 0 \\
Appeal to Fear & 1 & 1 & 0 & 2 & 0 \\
Appeal to Pity & 0 & 0 & 0 & 0 & 0 \\
Appeal to Ridicule & 8 & 1 & 1 & 4 & 5 \\
Appeal to Worse Problems & 3 & 0 & 0 & 0 & 1 \\
Causal Oversimplification & 2 & 2 & 1 & 4 & 2 \\
Circular Reasoning & 2 & 0 & 2 & 0 & 1 \\
Equivocation & 1 & 0 & 0 & 5 & 1 \\
False Analogy & 1 & 1 & 1 & 0 & 0 \\
False Causality & 3 & 4 & 2 & 1 & 2 \\
False Dilemma & 1 & 1 & 0 & 1 & 2 \\
Hasty Generalization & 4 & 2 & 3 & 5 & 3 \\
Slippery Slope & 1 & 1 & 0 & 7 & 1 \\
Straw Man & 2 & 5 & 0 & 0 & 3 \\
Fallacy of Division & 3 & 0 & 0 & 0 & 0 \\
Ad Hominem & 4 & 1 & 3 & 2 & 4 \\
Ad Populum & 3 & 1 & 0 & 5 & 1 \\
Appeal to (False) Authority & 0 & 2 & 1 & 3 & 1 \\
Appeal to Nature & 0 & 1 & 0 & 0 & 0 \\
Appeal to Tradition & 1 & 1 & 1 & 2 & 2 \\
Guilt by Association & 1 & 3 & 1 & 1 & 1 \\
Tu Quoque & 0 & 1 & 2 & 0 & 0 \\
Unknown & 0 & 0 & 0 & 0 & 0 \\ \bottomrule
\end{tabular}
\caption{Fallacies distribution at Level 2 of User 1, User 2, User 3, User 4, and the sample gold standard}\label{tab:users_distribution_fallacies_level_2}
\end{table*}




\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 1_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{User 1}}
        \label{fig:correct_fallacy_user_1_level_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 2_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{User 2}}
        \label{fig:correct_fallacy_user_2_level_1}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 3_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{User 3}}
        \label{fig:correct_fallacy_user_3_level_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 4_Level 1.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 1 for the \textbf{User 4}}
        \label{fig:correct_fallacy_user_4_level_1}
    \end{subfigure}

    \caption{Accuracy of fallacy labeling for spans that \textbf{exactly match} the gold standard at Level 1 for the Users' annotations. \emph{Exact Span} corresponds to the number of spans correctly identified by the user, \emph{Exact Span and Correct Label} corresponds to the number of correctly labeled spans out of the correctly identified spans.}
    \label{fig:correct_fallacy_users_level_1}
\end{figure*}


\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 1_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{User 1}}
        \label{fig:correct_fallacy_user_1_level_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 2_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{User 2}}
        \label{fig:correct_fallacy_user_2_level_2}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 3_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{User 3}}
        \label{fig:correct_fallacy_user_3_level_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{img/exact_match_fallacies_per_fallacious_span_user 4_Level 2.pdf}
        \caption{Accuracy of fallacy labeling for spans that exactly match the gold standard at Level 2 for the \textbf{User 4}}
        \label{fig:correct_fallacy_user_4_level_2}
    \end{subfigure}

    \caption{Accuracy of fallacy labeling for spans that \textbf{exactly match} the gold standard at Level 2 for the Users' annotations. \emph{Exact Span} corresponds to the number of spans correctly identified by the user, \emph{Exact Span and Correct Label} corresponds to the number of correctly labeled spans out of the correctly identified spans.}
    \label{fig:correct_fallacy_users_level_2}
\end{figure*}



==> MAFALDA_arXiv_-_Copie/src/evaluation_metric.tex <==
\subsection{Disjunctive Annotation Scheme}\label{sec:annotation}
\label{sec:metrics}

Before presenting our annotation scheme, we need to establish some common ground:

\begin{mydef}[label={def:text}]{Text}
    A text is a sequence of sentences $st_1, \ldots, st_n$.
\end{mydef}

\noindent A \emph{span} on a text is a contiguous sequence of sentences. The set $S$ of all spans of a text $st_1, \ldots, st_n$ is thus $S=\{st_i \ldots st_j \mid 0<i\leq j\leq n\}$. 

\begin{mydef}[label={def:span}]{Span}
The span of a fallacy in a text is the smallest contiguous sequence of sentences that comprises the conclusion and the premises of the fallacy.
If the span comprises a pronoun that refers to a premise or to the conclusion, that premise or conclusion is not included in the span.
\end{mydef}

\noindent We work on the level of sentences, 
because previous work has shown that agreement on the token level is even harder to achieve~\cite{jinLogicalFallacyDetection2022}. 
We allow the use of pronouns to decrease the size of the spans: When a sentence refers to another sentence by a pronoun, that other sentence does not have to be part of the span.
For instance, in Example (d) of Figure~\ref{fig:main}, the premise of the fallacy is in the title of the post, and the conclusion is at the end of the text. Thus, a span that covers the entire fallacy would have to cover the entire post from title to end. %
However, the pronoun ``This'' refers to the title, and thus we can omit the title from the span.
Nevertheless, %
a span can comprise several sentences. 

A span can be annotated with a label (such as a fallacy type) by an annotator (or a group of them) or by a system.
We now propose the key element of our disjunctive annotation scheme, in which subjectivity is not projected away, but explicitly embraced by allowing for several equally valid labels for the same span. 

\begin{mydef}[label={def:gold_standard}]{Gold Standard}
Let $\mathcal{F}$ be the set of fallacy types and $\bot$ be a special label that means ``no fallacy''.

Given a text and its set of spans $S$, %
a gold standard $G$ is a set of pairs of a span $s \in S$ and a set of labels from $\mathcal{F}\cup\{\bot\}$: %
\[G \subseteq S \times (\mathcal{P}(\mathcal{F}\cup\{\bot\})\setminus\{\emptyset, \{\bot\}\})\] %
Here, $\mathcal{P}(\cdot)$ denotes the powerset. 

\end{mydef}

\noindent 
The gold standard associates a given span with one or more fallacy labels. If more than one label is present, this means that any label is acceptable as an annotation. The gold standard can also associate a span with $\bot$, which means that the annotation of this span is optional. However, in this case, the gold standard has to associate the span also with at least one other label,
as we are not interested in annotating non-fallacious sentences. The gold standard can also contain the same span twice, which means that the span has to be annotated with two labels. 
The alternative labels for a span
can be generated through various methods during the annotation process, e.g.,~one annotator giving alternatives, a group of annotators proposing different labels due to lack of consensus, or multiple independent annotators combining their labels (see Example~\ref{ex:anno}).


















\noindent We define a prediction as the annotation of a text by a system or a user:

\begin{mydef}[label={def:prediction}]{Prediction}
Given a set of fallacy types $\mathcal{F}$, a text, and its set of spans $S$, a prediction $P$ is a set of pairs of a span $s\in S$ and a label $l\in\mathcal{F}$:
\[ P\subseteq S \times \mathcal{F}\] 
\end{mydef}
\noindent The following example gives substance to these definitions:
\begin{myexamplebox}[label={ex:anno}, breakable] %
Let ``$a\ b\ c\ d$'' be a text where $a$, $b$, $c$, and $d$ are sentences. 

Suppose \(S= \{a\ b, d\}\) (i.e.,~the sentences $a$ and $b$ are one fallacious span, and $d$ is a span of one fallacious sentence), $a\ b$ has labels $\{l_1, l_2\}$, and \(d\) has label \(\{l_3\}\).
In that case, \(G=\bigl\{ (a\ b, \{l_1, l_2\}) , (d, \{l_3\}) \bigl\}\)\\

An example of prediction $P$ could be $P=\{(a, l_1), (a, l_2), (b, l_3), (c, l_4),$ $(d, l_1)\}$
\end{myexamplebox}





\subsection{Evaluation Metrics.}



To compare two annotated spans, we %
adapt the precision and recall of \citet{martinoFineGrainedAnalysisPropaganda2019} to alternatives.
Given two spans, $p$ with its label $l_p$, and $g$ with its set of labels $l_g$, respectively, 
and a normalizing constant $h$, these metrics compute a comparison score as follows:
\[ C(p, l_p, g, l_g, h) = \frac{|p \cap g|}{h} \times \delta(l_p, l_g) \]
\noindent $\delta$ is a similarity function. We use 
$\delta(x,y)=[x \in y ]$, 
where $[\cdot]$ is the Iverson bracket.

Let $G$ be the gold standard, and let $P$ be the prediction of a user or a system.
The precision for $P$ is computed by comparing each span in $P$ against all spans in $G$, and taking the score of the best-matching one:
\[\textit{Precision}(P, G)\!=\!\!\frac{\sum\limits_{(p, l_p)\in P}\!
\max\limits_{(g, l_g)\in G}\!C(p, l_p, g, l_g, |p|)}{|P|}\]
\noindent If there are no annotations in $P$ (i.e., $|P|=0$), we set precision to 1. 
This choice is inspired by the intuition that a loss in precision should result only from false predictions. If there are no such false predictions, then precision should not be harmed.




To calculate the recall, we exclude all the spans from the gold standard that contain a $\bot$. The rationale for this choice is that %
when a span has also been marked as ``no fallacy'', its annotation is considered optional. Therefore, we do not want to 
penalize models that do not provide an annotation for such a span. %
We define the set $G^-$, which is $G$ restricted to the spans that do not map to $\bot$, i.e., 
$G^-=\{(s,L) \in G \mid \bot \notin L\}$. %
The recall is then computed as:
\[\textit{Recall}(P, G)\!=\!\!\frac{\sum\limits_{(g, l_g)\in G^-}\!
\max\limits_{(p, l_p)\in P}\!C(p, l_p, g, l_g, |g|)}{|G^-|}\]
\noindent %
If  $|G^-|=0$, we set the recall to 1. 
The intuition is that a model should be penalized in recall only for the annotations it misses from the gold standard. If there are no such missed annotations, recall should not suffer. Appendix~\ref{app:metrics_edge_cases} shows how our metrics handle various edge cases.









The F1-score is computed as usual as the harmonic mean of precision and recall.
It is easy to see that our definitions of precision and recall fall back to the standard definitions if $G$ does not have alternatives and all spans comprise only a single sentence. 
In that case, the score $C$ is 1 if the spans are identical and identically labeled.  %
If there are no alternatives, our measures are also identical to the ones in %
\citet{martinoFineGrainedAnalysisPropaganda2019},
with one difference: we use the $\max$ instead of a sum in the definitions to select the best matching span. In this way, two neighboring spans with the same label do not achieve full precision or recall if the gold standard requires one contiguous span with that label. Using $\max$ instead of a sum also avoids the case where \citet{martinoFineGrainedAnalysisPropaganda2019}'s metric yields precision or recall scores exceeding one. This occurs when the gold standard contains overlapping spans with identical labels, affecting precision, or when the prediction includes such overlaps, affecting recall. %
However, their metric is equivalent to ours as long as (1) there are no alternatives in the gold standard, (2) 
neither the gold standard nor the prediction contains overlapping spans with the same label and (3) each span from the gold standard overlaps with at most one span with the same label from the predictions and vice versa. 
Examples, proofs, and further details are in Appendix~\ref{app:metrics}.



==> MAFALDA_arXiv_-_Copie/src/experiments.tex <==
\section{Experiments}\label{sec:xp}
We will now evaluate the ability of state-of-the-art LLM to detect the fallacies in our benchmark. Our benchmark is not intended for training or fine-tuning, and hence, we study a zero-shot setting with basic prompts.
We are interested in the task of fallacy detection and classification of a given text, i.e.,~the input is a text, and the output is a list of annotated spans.

\subsection{Settings}
We study ChatGPT as well as 12 open-source models, covering different model sizes (Table~\ref{tab:result:partial}).
We use a bottom-up approach to evaluate our models starting at Level~2 granularity and extrapolate labels for Levels~1 and 0 based on these predictions, as our dataset includes three levels of granularity.

We employ a basic prompting approach that presents the model with our definition of a fallacy, the instruction to annotate the fallacies, the list of fallacies without their definitions, the corresponding text example, and the sentence to be labeled.
The detailed prompt can be found in Appendix~\ref{app:prompt}. Our experiments are conducted at the sentence level; spans are formed by grouping consecutive sentences with the same label.
A significant challenge with generative models is their inconsistent format output. Thus, we deem an output correct if it includes the name of the correct fallacy (or a part of it).
Details about the models can be found in Appendix~\ref{app:models}. 

\subsection{Results}
\label{sec:results}

\begin{table}[!ht]
    \centering
    \small

    \resizebox{\columnwidth }{!}{
     \begin{tabular}{lccc}
        \toprule
        & \multicolumn{3}{c}{MAFALDA} \\
        \cmidrule(lr){2-4} %
        Model & F1 Level 0~\textsuperscript{*} & F1 Level 1~\textsuperscript{*} & F1 Level 2\\
        \midrule
        Baseline random & 0.435 & 0.061 & 0.010  \\
        \midrule
        Falcon 7B& 0.397 & 0.130 & 0.022 \\
        LLAMA2 Chat 7B& 0.572 & 0.114 & 0.068 \\
        LLAMA2 7B& 0.492 & 0.148 & 0.038 \\
        Mistral Instruct 7B & 0.536 & 0.144 & 0.069 \\
        Mistral  7B & 0.450 & 0.127 & 0.044 \\
        Vicuna 7B & 0.494 & 0.134 & 0.051 \\
        WizardLM 7B & 0.490 & 0.087 & 0.036 \\
        Zephyr 7B & 0.524 & 0.192 & 0.098 \\
        LLaMA2 Chat 13B & 0.549 & 0.160 & 0.096 \\
        LLaMA2 13B & 0.458 & 0.129 & 0.039 \\
        Vicuna 13B & 0.557 & 0.173 & 0.100 \\
        WizardLM 13B & 0.520 & 0.177 & 0.093 \\
        \midrule
        GPT 3.5 175B & \textbf{0.627} & \textbf{0.201} & \textbf{0.138} \\
        \midrule
        Avg. Human & \textbf{0.749} & \textbf{0.352} & \textbf{0.186}\\
        on Sample & & & \\
        \bottomrule
    \end{tabular}
    }
    \begin{minipage}{\textwidth}
        \footnotesize
        \textsuperscript{*} Labels were extrapolated from Level 2.\\
    \end{minipage}
    \caption{Performance results of different models across different granularity levels in a zero-shot setting. Avg. human on sample concerns only the 20 subsamples of MAFALDA for the user study. Metrics are explained in Section~\ref{sec:metrics}.\label{tab:result:partial}}
    
\end{table}
    
Table \ref{tab:result:partial} shows the results across different granularity levels in a zero-shot setting, as evaluated using our metric (see Section~\ref{sec:metrics}). 
We added \textit{Baseline random}, a dummy model that predicts labels randomly following a uniform distribution.







At all levels of granularity, all models surpass the performance of the baseline model (except for Falcon on Level 0), indicating that they are successfully identifying certain patterns or features.
GPT~3.5 outperforms all other models at all levels. 
At Level 1, Zephyr 7B achieves comparable results to GPT 3.5, possibly thanks to the quality of its training dataset and/or engineering tricks, challenging the assumption that larger models are always more effective.
More surprisingly, LLaMA2 performs better in its 7B version than in its 13B version for Levels 0 and 1.
This phenomenon is in line with %
findings from \citet{DBLP:conf/emnlp/WeiKTL23}. 

We also investigate whether it makes a difference to prompt the models directly on Level 1 (as opposed to extrapolating Level~1 from Level~2). %
For Mistral Instruct and Zephyr, %
there is no significant difference: %
Mistral Instruct obtains an F1 score of 0.149, and Zephyr achieves an F1 score of 0.185.



\begin{table}[ht]
    \centering
    \small
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccc}
    \toprule
     Gold Standard & F1 Level 0~\textsuperscript{*} & F1 Level 1~\textsuperscript{*} & F1 Level 2 \\
    \midrule
    User 1 & 0.616 & 0.310 & 0.119 \\
    User 2 & 0.649 & 0.304 & 0.098 \\
    User 3 & 0.696 & 0.253 & 0.093 \\
    User 4 & 0.649 & 0.277 & 0.144 \\
    \midrule
    MAFALDA & \textbf{0.749} & \textbf{0.352} & \textbf{0.186} \\
    \bottomrule
    \end{tabular}
    }
    \begin{minipage}{\textwidth}
        \footnotesize
        \textsuperscript{*} Labels were extrapolated from Level 2.\\
    \end{minipage}
    \caption{Cross-comparison of user annotations and the gold standard. Each annotation of the user study has been alternatively used as a gold standard to demonstrate the superiority of our own gold standard.}
    \label{tab:user_gs}
\end{table}

We also measure human performance on our dataset (which constitutes, to our knowledge, the first such study in the fallacy classification literature).
We aim to establish (\textit{i}) whether humans outperform language models for the task at hand and (\textit{ii}) whether humans agree more with our gold standard than among themselves. %
As human effort is more costly than running a language model (and even more so since we need engaged annotators who do not resort to ChatGPT or other LLMs),
we asked four other annotators to annotate 20 randomly chosen examples on the same task as the systems.
On these 20 samples, we compared the results of human annotators and LLMs.
The low scores of human annotators reported in Table~\ref{tab:user_gs} show that the task is difficult.
Still, \textbf{human participants outperform the language models} as shown in Table~\ref{tab:result:partial}: 
Contrary to what previous work has demonstrated~\cite{gilardiChatGPTOutperformsCrowdWorkers2023}, GPT-3.5 does not perform better than humans. 

Next, we study whether they agree more with our gold standard than among themselves.
We treat each annotator's work as a gold standard and assess the precision, recall, and F1 scores of the other annotators. Our gold standard achieves an F1 score of 0.186 on average for humans (see Table~\ref{tab:user_gs}), outperforming the best alternative, which scores 0.144. More details about the annotators and the results are in Appendix~\ref{app:annotators} and~\ref{app:results}, respectively. 

We analyze the errors in the two models, GPT-3.5 and Falcon, focusing on their performance at Levels 1 and 2, alongside user study annotations. Our first goal is to determine whether the models, specifically the highest-performing GPT-3.5 and the lowest-performing Falcon, exhibit controlled or uncontrolled behavior in their output generation. 
While both models can produce nonsensical outputs, Falcon often predicts multiple irrelevant fallacies and significantly more unknown labels than GPT-3.5.

Our second goal is to determine which fallacy type is the most challenging. The analysis reveals that humans and models struggle with the fallacies of appeal to emotion. We hypothesize that emotions often appear in texts without necessarily constituting a fallacy, which complicates the distinction between emotional texts and fallacious texts that use appeals to emotion.
More details about this analysis are in Appendix~\ref{app:error_analysis}.










































==> MAFALDA_arXiv_-_Copie/src/intro.tex <==
\section{Introduction}\label{sec:intro}




%


A fallacy is an erroneous or invalid way of reasoning. 
Consider, e.g.,~the argument ``\textit{You must either support my presidential candidacy or be against America!}''. 
This argument is a \emph{false dilemma} fallacy: it wrongly assumes no other alternatives.
\textbf{Fallacies can be found in various forms of communication}, including speeches, advertisements~\cite{danciu2014manipulative}, Twitter/X posts~\cite{macagno2022argumentation}, and political debates~\cite{balalauStageAudiencePropaganda2021,goffredoFallaciousArgumentClassification2022}. 
They are also part of propaganda techniques employed to shape public opinion and promote specific agendas.
Most notably, fallacies 
played a role in the 2016 Brexit referendum~\cite{zappettini2019brexit}, 
and the debate about COVID-19 vaccinations~\cite{elsayed2020fallacies}, where fake news spread on news outlets and in social networks~\cite{martinoFineGrainedAnalysisPropaganda2019, sahaiBreakingInvisibleWall2021,balalauStageAudiencePropaganda2021}.
Detecting and identifying these fallacies is thus a task of broad importance. 

The recent advances in deep learning and the availability of more data have given rise to approaches for detecting and classifying fallacies in text automatically~\cite{martinoFineGrainedAnalysisPropaganda2019,al-omari-etal-2019-justdeep,balalauStageAudiencePropaganda2021,sahaiBreakingInvisibleWall2021,abdullahDetectingPropagandaTechniques2022}. 
And yet, this work is fragmented: \textbf{most approaches focus on specific types of corpora} (e.g.,~only speeches) or \textbf{specific types of fallacies} (e.g.,~only \emph{ad hominem} fallacies).
Furthermore, \textbf{not all works use the same types of fallacies}, 
there is no consensus on a common terminology~\cite{sep-fallacies}, and fallacies come at different levels of granularity: an \emph{appeal to emotion} can be, for instance, an \emph{appeal to anger}, \emph{fear}, \emph{pride}, or \emph{pity}. 
Most importantly, \textbf{annotating fallacies is an inherently subjective task}. While previous works acknowledge the subjectivity, none explicitly embraces it. %
On the contrary, the annotators typically aim for a unique annotation -- by discussion or vote. 
Additionally, \textbf{existing works do not give human performances} on the benchmarks and evaluate only models.


%

This paper addresses these drawbacks by introducing the Multi-level Annotated Fallacy Dataset MAFALDA -- a manually created fallacy classification benchmark. %
Our contributions are: 
\begin{enumerate}[noitemsep,nolistsep,leftmargin=4mm]
    \item A taxonomy of fallacies that aligns, consolidates, and unifies %
    existing public fallacy collections (Section~\ref{sec:def}).
    %
    \item A new annotation scheme -- coined disjunctive annotation scheme -- that accounts for the inherent subjectivity of fallacy annotation by permitting several correct annotations (Section~\ref{sec:annot_dataset}).
    %
    \item A corpus that merges existing corpora, with 9,545 non-annotated texts and 200 manually annotated texts with 260 instances of fallacies, each with a manual justification (Section~\ref{sec:dataset}).
    \item A study of the performance of state-of-the-art language models and humans on our benchmark (Section~\ref{sec:xp}). 
    % 
\end{enumerate}





\noindent %
All our code and data are publicly available under a CC-BY-SA license\footnote{as imposed by the dataset from
\citet{goffredoFallaciousArgumentClassification2022}} at %
\url{https://github.com/ChadiHelwe/MAFALDA}, allowing our study to be reproduced and built upon.
We start our paper by discussing related work in Section~\ref{sec:related_work}.






==> MAFALDA_arXiv_-_Copie/src/limitations.tex <==
\section*{Limitations}\label{sec:limitations}

Our work provides a dataset that may contain sensitive content such as racism, apologies for committing crimes, and misogyny. We believe that this is unavoidable in our fight against fake news and manipulative content. 

One limitation of our benchmark is that we may have been biased while annotating it. Our collective bias is limited because we come from diverse cultural backgrounds, countries, religions, and political convictions, but it may still exist. 
We have also made efforts to mitigate bias during our annotation, with clear guidelines, or by achieving a consensus or at least providing strong arguments in the form of a completed template as described in the formal definitions of Appendix~\ref{app:fallacy_list}. 

Our dataset has the potential for misuse in training systems that could be exploited for manipulative purposes, such as crafting more convincing fallacious arguments or disinformation campaigns.
Finally, models trained on this problem may wrongly label a text as fallacious. They must thus not be used to flag a text as fallacious without manual verification. %




A further consideration is the size of our dataset. It is relatively small due to the time-intensive nature of the annotation process. It is thus not suited for fine-tuning, but rather intended for evaluating large language models in zero-shot and few-shot settings.  %















==> MAFALDA_arXiv_-_Copie/src/related_work.tex <==

\begin{figure*}
\centering
\footnotesize
\begin{minipage}[b]{.49\textwidth}
\centering
\begin{subfigure}[b]{\linewidth}
  \centering
  \begin{tcolorbox}[boxrule=1pt,colback=white,colframe=mycustomcolor] %
  \textit{``\underline{We know God exists because he made everything.}''}
  \end{tcolorbox}
  \vspace{-1em}
  \caption{Circular Reasoning}
  \label{ex:implicit}
\end{subfigure}
\end{minipage}%
\hfill %
\begin{minipage}[b]{.49\textwidth}
\centering
\begin{subfigure}[b]{\linewidth}
  \centering
  \begin{tcolorbox}[boxrule=1pt,colback=white,colframe=mycustomcolor]
  \textit{if you had supported that attitude, we would not have won the Cold War. \underline{We won the Cold War because we invested and we}\\\underline{went forward.} (APPLAUSE.)}
  \end{tcolorbox}
  \vspace{-1em}
  \caption{Causal Oversimplification}
  \label{ex:political}
\end{subfigure}
\end{minipage}

\vspace{0.2cm} %

\begin{minipage}[b]{.49\textwidth}
\begin{subfigure}[b]{\textwidth}
  \centering
  \begin{tcolorbox}[boxrule=1pt,colback=white,colframe=mycustomcolor]
  \textit{``\underline{In the last New Hampshire primary election, my} \underline{favorite candidate won. Therefore, he will also win} \underline{the next primary election.}''}
  \end{tcolorbox}
  \vspace{-1em}
  \caption{Causal Oversimplification \textbf{OR} False Causality}
  \label{ex:main}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}[b]{.49\textwidth}
\begin{subfigure}[b]{\textwidth}
  \centering
  \begin{tcolorbox}[boxrule=1pt,colback=white,colframe=mycustomcolor]
``\textit{TITLE: Can I get into finance with a Law degree? POST: (...) \underline{This is law school arrogance at its finest.} \underline{Why not a brain surgeon?}}''
\end{tcolorbox}
  \vspace{-1em}
\caption{Appeal to Ridicule}
  \label{ex:finance_law_degree}
\end{subfigure}
\end{minipage}
\caption{Examples of Fallacies. The spans of the fallacies are \underline{underlined}. Example~\ref{ex:implicit} is from \citet{jinLogicalFallacyDetection2022}, \ref{ex:political}  from \citet{goffredoFallaciousArgumentClassification2022}, and \ref{ex:finance_law_degree} from \citet{sahaiBreakingInvisibleWall2021}. Detailed annotations are in Appendix~\ref{app:additional_examples}.
}
\label{fig:main}
\end{figure*}
\section{Related Work}\label{sec:related_work}

\subsection{Datasets}
Numerous works have created datasets of fallacies. 
\citet{habernalNameCallingDynamicsTriggers2018} created a dataset for \emph{ad hominem} fallacies from the ``Change My View'' subreddit. 
%
% 
\citet{martinoFineGrainedAnalysisPropaganda2019} created a news article dataset featuring 18 fallacies such as \emph{red herring, appeal to authority, bandwagon, etc.}.
% 
%
%
%
\citet{balalauStageAudiencePropaganda2021} trained models for propaganda technique identification using online forums.
% 
\citet{sahaiBreakingInvisibleWall2021} compiled a Reddit-based corpus for fallacy detection with eight types of fallacies.
%
% 
\citet{goffredoFallaciousArgumentClassification2022} introduced a dataset from American political debates with six different fallacy types. 
%
% 
Along the same line, \citet{jinLogicalFallacyDetection2022} curated a claim dataset, containing 13 types of fallacies, based on online quizzes and the Climate Feedback website, employing a novel approach that mimics first-order logic. %
% 
To address data annotation challenges, \citet{habernalArgotario2017} created the Argotario game for fallacy detection in QA pairs. It created a corpus of 5 fallacy types. 
% 
In the domain of (dis/mis)information, \citet{musiCOVID2022} and \citet{alhindiMultitask2022} annotated fallacies in COVID-19 and climate change articles with ten types of fallacies.
%
Lastly, \citet{payandeh2023susceptible} developed LOGICOM to evaluate large language models' (LLMs) robustness against logical fallacies in debate scenarios.
%

While all of these works advanced the understanding of fallacy detection, 
the studied fallacies are not the same across different works and are sometimes outright disjoint.
The only work that creates a comprehensive taxonomy of fallacies is the (not yet peer-reviewed) work of \citet{hong2023closer}. However, this work enumerates 232 fallacies, which is clearly too many to be handled by a human. And indeed, their dataset is composed only of toy examples generated by GPT-4.

%

In this paper, we propose a benchmark that not only unifies public datasets on fallacy detection 
in a handy yet all-embracing taxonomy, but also comes with human annotations, human explanations, and evaluations for both language models and humans.

\subsection{Subjectivity and Annotation Challenges} \label{subsec:subjectivity}

Human label variation is inherently part of annotating complex and subjective tasks~\cite{plank2022problem}. It is usually addressed with strategies such as simplifying the task, majority votes, or reconciliation of discrepancies. \citet{goffredoFallaciousArgumentClassification2022} computed the Krippendorff's $\alpha$ on a subset of fallacies and reached inter-annotator agreements (IAAs) ranging from 0.46 to 0.60, which is a moderate agreement. 
On simpler tasks such as identifying only \emph{ad hominem} using two groups of 6 workers, \citet{habernalNameCallingDynamicsTriggers2018} reported a Cohen's $\kappa$ of 0.79, which is a good agreement. However, they acknowledge the difficulty of annotated sub-categories such as \tuquoque~and \guiltbyassociation~(they found a low IAA, but the value is not provided). 
When annotating spans of propaganda techniques, a complex task, \citet{martinoFineGrainedAnalysisPropaganda2019} found a $\gamma$ IAA of 0.26, which is low. However, they could increase the IAA up to 0.60 when adding a reconciliation step. 
In \citet{sahaiBreakingInvisibleWall2021}, the annotator had to identify one fallacy at a time, and they reached a Cohen's $\kappa$ of 0.515 (ranging from 0.38 to 0.64 based on the fallacy), which is a moderate agreement. They also computed the $\gamma$ for the span selection per fallacy type and found values between 0.60 to 0.80, which is a good agreement. This was expected since it is a binary classification task.
\citet{sahaiBreakingInvisibleWall2021,jinLogicalFallacyDetection2022,musiCOVID2022,alhindiMultitask2022} used a reconciliation step too to tackle discrepancies in the annotations.

In summary, IAA in related work is usually only moderate. Disagreements are interpreted as noise, and are removed with various strategies. 
%
In this paper, we propose not just to acknowledge the subjectivity of fallacy annotation but actually to follow through with it.
We contend that there are cases 
where \textbf{multiple, equally valid annotations can coexist for the same textual span}. 
Therefore, we propose a new subjective annotation scheme that allows for several alternative labels for the same span. %



\subsection{Taxonomies of Fallacies}

Logical fallacies have been studied and classified since the time of Aristotle.
There is a notable diversity in approaches and contents across various sources. 
The works of Aristotle (see \citet{SophisticalRefutations2023}) and \citet{whatelyElementsLogic1897}, despite their historical significance, present limitations in terms of the breadth of fallacies covered, listing only 13 fallacies each (our work, in contrast, finds more than 20).
\citet{downesStephenGuideLogical} offers a more extensive list with 36 fallacies. However, it still fails to mention common fallacies such as \emph{appeal to nature}, \emph{appeal to tradition}, and \emph{guilt by association}. 
\citet{fallacyfiles} provides an exhaustive list of 87 fallacies. Yet, it provides only a rudimentary hierarchy (classifying, e.g., \emph{no true Scotsman} as a sub-category of \emph{equivocation}). 
 \citet{logicalfallacies} lists 48 fallacies -- but lacks a hierarchical framework altogether. 
At the other end of the spectrum, \citet{encycl_philo}, \citet{bennettLogicallyFallaciousUltimate2012}, \citet{hong2023closer}, and \citet{wiki_fallacies} offer extensive compilations of 231, 300+, 232, and 149 fallacies respectively. Yet, such a sheer volume of fallacies would be challenging in practical annotation tasks, as the annotator would have to scan (or memorize) hundreds of different fallacies.

Our work, in contrast, is driven by today's practical application scenarios. It aims to systematize and classify the fallacies used in current works on fallacy annotation, detection, and classification. 










==> MAFALDA_arXiv_-_Copie/src/taxonomy.tex <==
\subsection{Taxonomy of Fallacies}\label{sec:tax}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{img/vertical_taxonomy.pdf}
    \caption{Tree structure of our taxonomy. Detailed definitions of the fallacies are in Appendix~\ref{app:informal_def}.
    }
    \label{fig:taxonomy}
\end{figure*}








In this paper, we propose a taxonomy that unifies and consolidates all types of fallacies used in current work on fallacy detection. 
We built our taxonomy manually, starting with a collection of fallacy types that are used in related work. 
Since the same fallacy can appear in different datasets under different names, we aligned equivalent fallacies manually. %
We used the definitions and guidelines in the source datasets to determine whether two fallacies are equivalent.
We removed fallacies that were too broad (e.g.,~\emph{appeal to emotion} could cover many emotions), fallacies that appeared in only a single work (e.g.,~\emph{confusion fallacy} appears only in~\citet{martinoFineGrainedAnalysisPropaganda2019}), and we merged fallacies that were too similar in their definitions (like \emph{begging the question} and \emph{circular reasoning}).
Some fallacies were not taken into account because they were not actually fallacies in our definition. These are, e.g., rhetorical techniques such as
\emph{flag waving} or \emph{repetition}.
Our list can obviously be extended in the future with new fallacies. Details on how our collection unifies existing works are in Appendix~\ref{app:comparison_of_types}.

We grouped our fallacies into broader categories to create a taxonomy on top of our collection. 
We chose the categories that Aristotle originally proposed~\cite{wisse1989ethos}, %
because %
it has been shown to be applicable across various forms of communication -- from political speeches to advertisements~\cite{wisse1989ethos}. This yields the following taxonomy:
\begin{enumerate}[noitemsep,nolistsep,leftmargin=4mm]
    \item \textbf{Level 0} is a binary classification, categorizing text as either fallacious or non-fallacious.
    \item \textbf{Level 1} groups fallacies into Aristotle's categories: `Pathos' (appeals to emotion), `Ethos' (fallacies of credibility), and `Logos' (fallacies of logic, relevance, or evidence).
    \item \textbf{Level 2} contains fine-grained fallacies within the broad categories of Level 1.
          For instance, under \emph{fallacy of credibility}, we have specific fallacies such as \emph{appeal to tradition}, \emph{ad populum}, and \emph{guilt by association}.
\end{enumerate}
\noindent Our taxonomy is shown in Figure~\ref{fig:taxonomy}.
For each fallacy, we provide \textbf{both a formal and an informal definition} in Appendix~\ref{app:informal_def} (inspired by \citet{bennettLogicallyFallaciousUltimate2012}).
For instance, the \appealtoridicule{} is informally defined as ``an argument that portrays the opponent's position as absurd or ridiculous with the intention of discrediting it.''. 
Formally, it is defined as ``$E_1$ claims $P$. $E_2$ makes $P$ look ridiculous, by misrepresenting $P$ ($P$'). Therefore, $\neg P$.'', 
where $E_i$ are entities (e.g., people, organizations, etc.), and $P$ is a proposition.










